A Holomorphic perspective of Strict Deformation Quantization

We provide and discuss complex analytic methods for overcoming the formal character of formal deformation quantization. This is a necessity for returning to physically meaningful statements, and accounts for the fact that the formal parameter $\hbar$ carries the interpretation of Planck's constant. As formal star products are given by a formal power series, this naturally leads into the realm of holomorphic functions and analytic continuation, both in finite and infinite dimensions. We propose a general notion of strict deformation quantization and investigate how one can use established results from complex analysis to think about the resulting objects. Within the main body of the text, the outlined program is then put into practice for strict deformation quantizations of constant Poisson structures on locally convex vector spaces and the strict deformation quantization of canonical mechanics on the cotangent bundle of a Lie group. Numerous auxiliary results, many of which are well-known yet remarkable in their own right, are provided throughout.

==> sec_0TopologiesHolomorphic.tex <==
% !TeX root = ../Dissertation.tex

In this section, we study the images of the completion $\hat{\Sym}_0(V)$ under $\iota$. While the quite algebraic Gateaux holomorphy holds without further assumptions, we will have to make some to guarantee Fréchet holomorphy.



It might be worth looking into an alternative proof based on uniform convergence of the Taylor series.




\begin{example}[Sequence Spaces: Redux]
    We return to Example~\ref{ex:Sequences}. Let first $J \cong \field{N}$ be countable. As the Dirac functionals $\delta_n$ with $n \in \field{N}$ constitute a defining system for the product topology, $\field{C}^\field{N}$ is a Fréchet space and thus metrizable. \textcolor{red}{But this does not imply metrizability of $V'_\beta$!}
    By Theorem~\ref{thm:FrechetHolomorphy}, $\iota(a)$ is Fréchet holomorphic for every $a \in \Sym_0(\field{C}^\field{N})$. Conversely, as any bounded subset of $\field{C}^J$ generates a finite dimensional subspace, there is a countable fundamental system of bounded subsets for $\field{C}^J$ only if $J$ is countable itself. Let now $J$ be uncountable. The goal is to construct a non trivial Fréchet holomorphic $\iota(a)$ beyond the countable case. To this end, let $J_n = \big\{j_m^{(n)} \;|\; m \in \field{N}\big\} \subseteq J$ be countable, pairwise disjoint subsets of $J$. We define
    \begin{equation}
        a^{(n)}_{k_1 \cdots k_n}
        \coloneqq
        \begin{cases}
            \frac{1}{n!}
            \frac{1}{2^{m_1 + \cdots + m_n}}
            &\; \textrm{if} \;
            k_1 = j_{m_1}^{(n)}, \ldots, k_n = j_{m_n}^{(n)} \\
            0
            &\; \textrm{else}
        \end{cases}
    \end{equation}
    for all $n \in \field{N}$ and $j_1, \ldots, j_n \in J$. By construction, the resulting sequences $a^{(n)} \in \field{C}^{J^n}$ are invariant under permutation of the indices, i.e. actually come from symmetric tensors, see again \eqref{eq:SequenceSpacePower}. Notice that for each $j \in J$, we have $j \in J_n$ for at most one $n \in \field{N}$. Consequently, at most one term in \eqref{eq:SequenceSpaceSummability} for $a \coloneqq \sum_{n=0}^{\infty} a^{(n)}$ does not vanish, i.e. $a \in \Sym_0(\field{C}^J)$. By Lemma~\ref{lem:Gateaux}, $\iota(a)$ is hence Gateaux holomorphic. The idea for the local boundedness is that $a$ happens to have summable coefficients in both ``directions''. A bit more precise, we note for $c \ge 0$
    \begin{equation*}
        \sum_{n=0}^\infty
        c^n
        \sum_{k_1, \ldots, k_n \in J}
        \abs[\big]{a_{k_1 \cdots k_n}^{(n)}}
        =
        \sum_{n=1}^\infty
        c^n
        \sum_{m_1, \ldots, m_n = 1}^\infty
        \frac{1}{n!}
        \frac{1}{2^{m_1 + \cdots + m_n}}
        =
        \sum_{n=1}^\infty
        \frac{c^n}{n!}
        \le
        \exp(c)
        <
        \infty.
    \end{equation*}
    Let now $\gamma_0 \in \field{C}^{(J)}$ and consider the $\ell^\infty$-ball $\Ball_{\supnorm{\argument}, 1}(\gamma_0) \subseteq \field{C}^{(J)}$, which is an open neighbourhood of $\gamma_0$. Let $M \coloneqq \max_{j \in J} \abs{\gamma_j} + 1$. From \eqref{eq:SequenceSpaceIotaSeries}, we obtain the estimate
    \begin{equation*}
        \abs[\bigg]
        {\iota(a) \at[\Big]{\gamma}}
        \le
        \sum_{n=0}^\infty
        \sum_{j_1, \ldots, j_n \in J}
        \abs[\big]{a_{j_1 \cdots j_n}^{(n)}}
        M^n
        <
        \infty
    \end{equation*}
    for $\gamma \in \Ball_{\supnorm{\argument}, 1}(\gamma_0)$. Hence $\iota(a)$ is locally bounded and hence Fréchet holomorphic by \cite[Prop.~3.7]{dineen:1999a}. Thus, the conditions in Theorem~\ref{thm:FrechetHolomorphy} are not necessary at all. However, the trick with the summability already implies that at most countably many coefficients are nonvanishing in each order $n$, as the relevant series would diverge otherwise.
    %    Next, we construct a function of drastically different nature: One that is not locally bounded at $0$ and hence not Fréchet holomorphic. To this end, we keep the sets $J_n$ and define
    %    \begin{equation}
        %        b^{(n)}_{k_1 \cdots k_n}
        %        \coloneqq
        %        \begin{cases}
            %            1
            %            &\; \textrm{if} \;
            %            k_1, \ldots, k_n \in J_n \\
            %            0
            %            &\; \textrm{else}
            %        \end{cases}
        %    \end{equation}
    %    for all $n \in \field{N}$. As before, we have $b \coloneqq \sum_{n=1}^{\infty} b^{(n)} \in \Sym_0(\field{C}^J)$. Let $U \subseteq \field{C}^{(J)}$ be an open neighbourhood of zero. Then there exist seminorms $\seminorm{p}_j$ on $\field{C}$ such that $\Ball_{\seminorm{p},1}(0) \subseteq U$, where $\seminorm{p} = \sum_{j \in J} \seminorm{p}_j$ as usual. If there are $n \in \field{N}$ and $j \in J_n$ such that $\ker \seminorm{p}_j \neq \{0\}$, then $m \basis{e}_j \in \Ball_{\seminorm{p},1}(0)$ and by \eqref{eq:SequenceSpaceIotaSeries}  $\iota(b) \at{m \basis{e}_j} = m^n$ for all $m \in \field{N}$. Hence $\iota(b)$ is unbounded on $U$. Otherwise, each $\seminorm{p}_j$ is a norm on $\field{C}$, wherefore there are corresponding $c_j > 0$ such that $\abs{z} \ge c_j \seminorm{p}_j(z)$ for all $z \in \field{C}$. That is, the circles $\disk_{c_j} \subseteq \Ball_{\seminorm{p},1}(0)$ for all $j \in J$. In particular, the sequences $\gamma_n \coloneqq \tfrac{1}{2} \sum_{m=1}^{n} c_{j_m} e_{j_m} \in U$.
    %
    %    Even worse, consider $v \in \field{C}^J$ with $v_j = 1$ for all $j \in J$. Then what we have shown yields
    %    \begin{equation*}
        %        \iota_1(v)
        %        \at[\Big]{\gamma_n}
        %        =
        %        \sum_{m=1}^\infty
        %        \gamma_{j_m}
        %        =
        %        \frac{1}{2}
        %        \sum_{m=1}^n
        %        c_{j_m},
        %    \end{equation*}
    %    which might be convergent and hence bounded.
\end{example}






\begin{proposition}
    Check when $V'_\beta$ is bornological. In this case, Fréchet holomorphy (via local boundedness) follows from boundedness on bounded subsets, see Dineen.
\end{proposition}


Having established various criteria for Fréchet holomorphy, the following question is immediate: Is the image of our mapping $\iota$ exactly the space of holomorphic functions of bounded type on $V'_\beta$?
